Tensor-Krylov method for computing eigenvalues of parameter-dependent matrices

In this paper we extend the Residual Arnoldi method for calculating an extreme eigenvalue (e.g. largest real part, dominant,...) to the case where the matrices depend on parameters. The difference between this Arnoldi method and the classical Arnoldi algorithm is that in the former the residual is added to the subspace. We develop a Tensor-Krylov method that applies the Residual Arnoldi method (RA) for a grid of parameter points at the same time. The subspace contains an approximate Krylov space for all these points. Instead of adding the residuals for all parameter values to the subspace we create a low-rank approximation of the matrix consisting of these residuals and add only the column space to the subspace. In order to keep the computations efficient, it is needed to limit the dimension of the subspace and to restart once the subspace has reached the prescribed maximal dimension. The novelty of this approach is twofold. Firstly, we observed that a large error in the low-rank approximations is allowed without slowing down the convergence, which implies that we can do more iterations before restarting. Secondly, we pay particular attention to the way the subspace is restarted, since classical restarting techniques give a too large subspace in our case. We motivate why it is good enough to just keep the approximation of the searched eigenvector. At the end of the paper we extend this algorithm to shift-and-invert Residual Arnoldi method to calculate the eigenvalue close to a shift $\sigma$ for a specific parameter dependency. We provide theoretical results and report numerical experiments. The Matlab code is publicly available.

==> Tables/random_subspace_3.tex <==
\begin{center}
\begin{tabular}{|l|l|l|}  
\hline
&Average dimension of subspace &nbr of herstarts \\\hline
$\epsilon_W =0.1$&71.83&17\\\hline
$\epsilon_X=1e-12, \epsilon_W =0.001$&79.66&23\\\hline
$\epsilon_X=1e-12, \epsilon_W =1e-07$&106.04&24\\\hline
$\epsilon_X=1e-12, \epsilon_W =1e-09$&117.19&24\\\hline
\end{tabular}
\end{center}
\caption{Table with statistics about the subspace for the example in Figure \ref{fig:random_results} (a). The tolerance $\epsilon_X$ is always $10^{-12}$ and the maximal dimension of the subspace is $100$. We see that when taking a high value for $\epsilon_W$ the average dimension is less high and that we need to restart less times.} \label{tab:random_subs_3}
% This file was created in matlab file figures_random on 15-Oct-2019

==> Tables/random_subspace_4.tex <==
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
&Average size of subspace &nbr of herstarts \\\hline
$\epsilon_X=1e-12, \epsilon_W =0.1$&64.03&10\\\hline
$\epsilon_X=1e-12, \epsilon_W =0.001$&67.37&15\\\hline
$\epsilon_X=1e-12, \epsilon_W =1e-07$&74.75&23\\\hline
$\epsilon_X=1e-12, \epsilon_W =1e-09$&81.92&24\\\hline
\end{tabular}
\end{center}
\caption{Table with statistics about the subspace for the example in Figure \ref{fig:random_results} (c). We see that when taking a high value for $\epsilon_W$ the average dimension is less high and that we need to restart less times.} \label{tab:random_subs_4}
% This file was created in matlab file figures_random on 15-Oct-2019

==> Tables/table_conv_diff1.tex <==
\begin{center}
\begin{tabular}{|l|l|l|l|l|}
\hline
&$\epsilon_X=10^{-3},$ &$\epsilon_X=10^{-12},$ &$\epsilon_X=10^{-3},$ &$\epsilon_X=10^{-12},$ \\
&$\epsilon_W =10^{-3}$ & $\epsilon_W =10^{-3}$ & $ \epsilon_W =10^{-12}$ & $ \epsilon_W =10^{-12}$ \\\hline
nbr. restarts&47&63&85&151\\\hline
Avg. size of subspace&90.2675&89.2&91.0325&100.3413\\\hline
nbr. matrix-vector prod. (line \ref{line:AX_1})&26566&36230&48484&94240\\\hline
nbr. matrix-vector prod. (line \ref{line:A(X)})&11574&37436&10960&37340\\\hline
\end{tabular}
\end{center}
\caption{ Example \ref{ex:conv_diff}: Statistisc about the experiments to see the effect of $\epsilon_W$ and $\epsilon_X$. We see that the average size of the subspace is not influenced by the chosen tolerances $\epsilon_X$ and $\epsilon_W$. This means that the cost of calculating eigenvalues of the projected problem stay the same. We observe that the number of matrix-vector products in line \ref{line:AX_1} resp. \ref{line:A(X)} is influenced by the tolerance $\epsilon_X$ resp. $\epsilon_W$.}
% This file was created in matlab file table_conv_diff on 04-Nov-2019

==> Tables/table_conv_diff_vartol.tex <==
\begin{center}
\begin{tabular}{|l|l|l|l|l|}
\hline
&$\epsilon_X=10^{-3}$ &$\epsilon_X=10^{-12}$ &$\epsilon_X=10^{-3}$ &$\epsilon_X=10^{-12}$ \\
& $\epsilon_R =5 \times 10^{-4}$ & $\epsilon_R =5 \times 10^{-4}$ & $\epsilon_R =5 \times 10^{-13}$ & $\epsilon_R =5 \times 10^{-13}$ \\\hline
Avg. number of inner products&1429.9167&2574.2233&3434.36&11358.56\\
for reduced eigenvalue problem & & & & \\\hline
\end{tabular}
\end{center}
\caption{test tabel}
% This file was created in matlab file table_conv_diff on 18-Feb-2020
